Multidimensional Online Resource Allocation for Large Language Model Services under Nonstationary Demand

We study multidimensional online generalized assignment under nonstationary arrivals, motivated by resource allocation for large language model agent services. Providers may commit model and tool allowances to agent tasks upon admission, reserving budgets for their internal execution loops. Each request is rejected or accepted with an irrevocable assignment to one compatible server, earning reward and consuming a vector of its nonreplenishing budgets. Arrivals are independent with known, potentially time-varying type distributions. Scalar reductions can discard feasible combinations of requests with complementary resource requirements. To maximize expected reward, we develop Vector-Aware Best-Fit, which combines linear-programming-guided candidate routing with calibrated acceptance while retaining vector feasibility. Relative to the expected clairvoyant offline optimum, its guarantee improves on scalar reduction in the multidimensional case and has the best possible inverse-dimensional order. With an appropriate acceptance parameter, the proposed policy attains the optimal competitive ratio on all-heavy instances, where every feasible assignment consumes more than half of at least one resource budget. We further develop two heuristics that retain its performance guarantee. Computational results show that the heuristics perform well against benchmarks in most tested settings, especially when capacity is scarce relative to demand.

==> macro.tex <==
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{nicefrac}
\newcommand{\samp}{\textsc{Sam}}
\newcommand{\samr}{\textsc{Sam$\gamma$}}
\newcommand{\samcr}{\textsc{Col$\gamma$}}
\newcommand{\samc}{\textsc{Col}}
\newcommand{\sth}{\textsc{Sam+}}
\newcommand{\cth}{\textsc{Col+}}
\newcommand{\st}{\textsc{Sth}}
\newcommand{\ct}{\textsc{Cth}}
\newcommand{\hg}{\textsc{HG}}

\newcommand{\grd}{\textsc{Grd}}
\newcommand{\rcp}{\textsc{Rcp}}
\newcommand{\bat}{\textsc{Bat}}
\newcommand{\p}{{p}}
\newcommand{\tv}{{n}}
\newcommand{\Ed}{{D}}
\newcommand{\Dist}{\mathbb{D}}
\newcommand{\s}{s}

\newcommand{\density}{{q}}
\newcommand{\pmin}{P^G}
\newcommand{\nmax}{N^B}
\newcommand{\lammax}{D^P}
\newcommand{\uvar}{\Delta}
\newcommand{\dmin}{\text{D}_{\text{min}}}
\newcommand{\dmax}{\text{D}_{\text{max}}}
\newcommand{\Bin}{{B}}

\newcommand{\Constraint}{Constr.}
\newcommand{\mulset}{J}

\newenvironment{Proof}[1][Proof]
{{\par\noindent \it #1.\quad}}{\hfill $\square$\par}

